Flying Hand: End-Effector-Centric Framework for Versatile Aerial Manipulation Teleoperation and Policy Learning

Aerial manipulation has recently attracted increasing interest from both industry and academia. Previous approaches have demonstrated success in various specific tasks. However, their hardware design and control frameworks are often tightly coupled with task specifications, limiting the development of cross-task and cross-platform algorithms. Inspired by the success of robot learning in tabletop manipulation, we propose a unified aerial manipulation framework with an end-effector-centric interface that decouples high-level platform-agnostic decision-making from task-agnostic low-level control. Our framework consists of a fully-actuated hexarotor with a 4-DoF robotic arm, an end-effector-centric whole-body model predictive controller, and a high-level policy. The high-precision end-effector controller enables efficient and intuitive aerial teleoperation for versatile tasks and facilitates the development of imitation learning policies. Real-world experiments show that the proposed framework significantly improves end-effector tracking accuracy, and can handle multiple aerial teleoperation and imitation learning tasks, including writing, peg-in-hole, pick and place, changing light bulbs, etc. We believe the proposed framework provides one way to standardize and unify aerial manipulation into the general manipulation community and to advance the field. Project website: https://lecar-lab.github.io/flying_hand/.

==> 7Experiment.tex <==
\section{Experiment: Trajectory Tracking}
\label{sec: experiment-tracking}

\guanqi{update DH params}

\subsection{Experiment Setup}
To show the effectiveness of our proposed method, we perform a comparison between our control methods against two baseline approaches:
\guanqi{comparsion study}

\begin{enumerate} 
\item \textbf{w.o. MPC}: This baseline disregards both the fully-actuated UAV and arm dynamics, relying solely on inverse kinematics (IK) for motion planning. The UAV follows the desired trajectory generated by the IK planner using a feedback controller from \citep{guo2024flyingcalligraphercontactawaremotion}. 
\item \textbf{w.o. L1}: This baseline excludes the L1 adaptive component, leaving disturbances from UAV-manipulator interactions and modeling uncertainties uncompensated during control execution. 
\end{enumerate}


We conduct experiments with three types of reference trajectories for the end-effector, each lasting 60 seconds. The setpoint trajectory requires the aerial manipulator to keep the end-effector hovering at a fixed position. The ellipse trajectory requires tracking a sinusoidal trajectory defined as $(x, y, z) = [0.5\sin(0.3t), 0.0, 1.4+0.2\sin(0.3t+0.75)]$. The figure-8 trajectory requires to track a trajectory $(x, y, z) = [0.1 + 0.6\sin(0.3t), 0.0, 1.35+0.25\sin(0.6t)]$. The maximum velocity in the reference trajectory is about $0.2$ m/s. The pitch, row and yaw attitude of the end-effector is fixed at zero during the tracking.

\guanqi{3 time repeat, how to compute metrics, explain violin plot (how to draw)}

\subsection{Implementation Details}

\guanqi{more details about hardware and perception}

The optimal control problem in the EE-centric MPC is implemented using ACADOS~\citep{Verschueren2021} with a $25$ms discretisation step and a $2.5$s constant prediction horizon, running in $100$ Hz, and other controller parameters are listed in Table \ref{tab:mpc_param}. The control output is executed in a receding horizon style, where at each iteration, only the first control input $\bm u_0$ is applied to the system.

\begin{table}[t]
\centering
\caption{\textbf{Controller Parameters}}
\label{tab:mpc_param}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l p{5.5cm}}
\toprule
Horizon Length $T$ & $2.5$ s \\
Horizon Steps $N$ & $100$ \\
State Cost $\bm{Q}_p$ & $\mathrm{diag}(12, 12, 12)$ \\
Rotation Cost $\bm{Q}_R$ & $\mathrm{diag}(10, 10, 10)$ \\
Velocity Cost $\bm{Q}_v$ & $\mathrm{diag}(0.1, 0.1, 0.1)$ \\
Joint Angle Cost $\bm{Q}_\theta$ & $\mathrm{diag}(0.1, 0.1, 0.1)$ \\
Control Cost $\bm{Q}_u$ & $\mathrm{diag}(0.03, 0.03, 0.03, 0.1, 0.1, 0.1)$ \\
\bottomrule
\end{tabular}
\end{table}


Since both the L1 adaptive controller and the MPC controller require accurate system modeling $\bm f_{dyn}$ to achieve effective control performance, we perform system identification to estimate uncertain parameters shown in Table \ref{tab:sysid}.
We excite the system with two types of motions. First, arm motion-only trajectories are executed while keeping the UAV stationary to calibrate the DH parameters $\bm \zeta$ and joint servo delay $\bm\beta$. These trajectories ensure that the manipulator kinematic parameters and joint motor dynamics accurately reflect the actual manipulator motion response. Second, UAV free-flight trajectories are conducted to identify the drone dynamics described in Eq. \eqref{uav_dyn}.


\begin{table}[t]
\centering
\caption{\textbf{System Identification Results}}
\label{tab:sysid}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l p{5.5cm}}
\toprule
Mass Matrix $\bm{M}$ & $\mathrm{diag}(0.105, 0.121, 0.101, 0.025, 0.011, 0.013)$ \\
Motor Delay $\beta$ & ($0.66$, $0.68$, $0.81$, $0.85$) \\
Joint 1 DH Param $\bm \zeta_1$& $d_1 = 0.0$, $a_1 = 0.363$, $\alpha_1 = 0.10$ \\
Joint 2 DH Param $\bm \zeta_2$ & $d_2 = 0.050$, $a_2 = 0.441$, $\alpha_2 = -0.10$ \\
Joint 3 DH Param $\bm \zeta_3$ & $d_3 = 0.0$, $a_3 = 0.007$, $\alpha_3 = -1.578$ \\
Joint 4 DH Param $\bm \zeta_4$ & $d_4 = 0.076$, $a_4 = 0.200$, $\alpha_4 = 0.0$ \\
\bottomrule
\end{tabular}
\end{table}







\subsection{Trajectory Tracking}


The trajectory tracking experiment demonstrates that our proposed method achieves the lowest tracking error, with approximately 1 cm in hover and 4 cm during motion (Table \ref{tab:tracking}). In comparison, the w.o. L1 baseline exhibits 1.3 cm and 6.5 cm, respectively, while the w.o. MPC baseline performs the worst, with 2 cm in hover and 10 cm in motion. The increased tracking error during motion is primarily due to the complex interaction between the UAV and the manipulator, where simultaneous movement introduces dynamic coupling effects that make precise tracking more challenging.

As illustrated in Fig. \ref{fig: tracking}, our method (blue) demonstrates the best tracking performance. The w.o. L1 baseline (green) exhibits overshoot in the X and Z axes and bias in Y, indicating that the L1 controller effectively mitigates both transient and steady-state errors caused by model uncertainties. The w.o. MPC baseline (orange) suffers from significant motion lag, as its inverse kinematics fail to account for UAV dynamics. The error distributions in Fig. \ref{fig: err_dist} further validate these findings, showing that our method achieves the smallest and most centered error, whereas the L1 baseline exhibits steady-state errors and the MPC baseline displays a broader error spread due to dynamic lag. These results confirm the effectiveness of our proposed control scheme. 

Despite the high tracking performance, there is still room for improvement. Fig. \ref{fig: x-z} reveals that tracking error increases at lower altitudes (~1m), likely due to unmodeled ground and wall effect disturbances. Additionally, oscillations in the end-effector trajectory are observed across all methods. We notice servo backlash (around $0.5^\circ$ dead zone), which results in a 2 cm control dead zone in the end-effector task space, limiting tracking precision during fast UAV maneuvers. Further improvements can be achieved through more accurate system modeling and higher-precision hardware to enhance tracking accuracy.

\begin{table}[t]
\centering
\caption{End-Effector Trajectory tracking performance}
\label{tab:tracking}
\begin{tabular}{lcccc}
\toprule
RMSE(cm) & Setpoint & Ellipse & Figure-8 &  \\
\midrule
Our Method & \textbf{1.00 $\pm$ 0.11} & \textbf{3.98 $\pm$ 0.41} & \textbf{4.62 $\pm$ 0.58}\\
w.o. L1 Adaptation & 1.33 $\pm$ 0.16 & 6.67 $\pm$ 0.42 & 6.28 $\pm$ 0.50 \\
w.o. MPC &  2.07 $\pm$ 0.19 & 11.25 $\pm$ 0.83 & 9.64 $\pm$ 1.07 \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/control/fig1_plot.pdf}
    \caption{End-effector tracking performance of aerial manipulator using three methods in Figure-8 trajectory.}
    \label{fig: tracking}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/control/fig2_plot.pdf}
    \caption{End-effector tracking error distribution using three methods.
    }
    \label{fig: err_dist}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=1.01\linewidth]{Figure/control/fig3_plot.pdf}
    \caption{Comparison of Figure-8 and Ellipse trajectory tracking performance across three methods.}
    \label{fig: x-z}
\end{figure}

